CRWIZ: A Framework for Crowdsourcing Real-Time Wizard-of-Oz Dialogues

Large corpora of task-based and open-domain conversational dialogues are hugely valuable in the field of data-driven dialogue systems. Crowdsourcing platforms, such as Amazon Mechanical Turk, have been an effective method for collecting such large amounts of data. However, difficulties arise when task-based dialogues require expert domain knowledge or rapid access to domain-relevant information, such as databases for tourism. This will become even more prevalent as dialogue systems become increasingly ambitious, expanding into tasks with high levels of complexity that require collaboration and forward planning, such as in our domain of emergency response. In this paper, we propose CRWIZ: a framework for collecting real-time Wizard of Oz dialogues through crowdsourcing for collaborative, complex tasks. This framework uses semi-guided dialogue to avoid interactions that breach procedures and processes only known to experts, while enabling the capture of a wide variety of interactions. The framework is available at https://github.com/JChiyah/crwiz

==> README <==
KNOWN ISSUES

Even if the compilation is successful, on overleaf the following error message appears during (re)compilation:
===ERROR MESSAGE BEGINNING===
 /usr/local/texlive/2018/texmf-dist/tex/latex/base/ts1enc.dfu, line 115
Missing number, treated as zero.

<to be read again> 
                   F
l.115 ...icodeCharacter{FEFF}{\ifhmode\nobreak\fi}
                                                  
A number should have been here; I inserted `0'.
(If you can't figure out why I needed to see a number,
look up `weird error' in the index to The TeXbook.)
===ERROR MESSAGE END===

